Fashionpedia-Ads: Do Your Favorite Advertisements Reveal Your Fashion Taste?

Consumers are exposed to advertisements across many different domains on the internet, such as fashion, beauty, car, food, and others. On the other hand, fashion represents second highest e-commerce shopping category. Does consumer digital record behavior on various fashion ad images reveal their fashion taste? Does ads from other domains infer their fashion taste as well? In this paper, we study the correlation between advertisements and fashion taste. Towards this goal, we introduce a new dataset, Fashionpedia-Ads, which asks subjects to provide their preferences on both ad (fashion, beauty, car, and dessert) and fashion product (social network and e-commerce style) images. Furthermore, we exhaustively collect and annotate the emotional, visual and textual information on the ad images from multi-perspectives (abstractive level, physical level, captions, and brands). We open-source Fashionpedia-Ads to enable future studies and encourage more approaches to interpretability research between advertisements and fashion taste.

==> main/sec3_dataset.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{images/ontology_compressed.pdf}
\caption{Ontology visualization. We select 28 labels from a general human motive taxonomy used in psychology research~\cite{motiveTaxonomy2017}. There are 9 super-categories in total \textit{(in black box)}, namely ``virtues'', ``self-fulfill'', ``openness to experience'', ``security and belonging'', ``power'', ``health'', ``family'', ``ambition and ability'', ''financial and occupational success''. 
See the Appendix~\ref{supsec:data_analysis} for dataset statistics.
}
\label{fig:ontology}
% \vspace{-0.2cm}
\end{figure*}

\section{Intentonomy Dataset}
\label{sec: anno}



\paragraph{Images}
Our dataset is built up of free-licensing high-resolution photos from the website Unsplash\footnote{\href{https://unsplash.com/data}{Unsplash Full Dataset 1.1.0}}.
We sample images with common keywords that are similar to social media hashtags, including ``people'',``happy'', \etc. 
The resulting images cover a wide range of everyday life scenes (\eg, from parties, vacations, and work).

\cvpara{Intent taxonomy}
The selection of intent labels is a non-trivial exercise. The labels must form a representative set of motives\footnote{We use \emph{intent} and \emph{motive} interchangeably} 
from social media posts, and it should occur with high enough frequencies in the collection of the dataset.
Previous work on motive taxonomies~\cite{motiveTaxonomy2017} provide a solid foundation for our study.
However, not all of the 161 human motives presented in~\cite{motiveTaxonomy2017} are suitable in the context of social media posts, or can be inferred from single-image inputs.
For example, one might need background information about the person inside the image to judge if the intent is ``being spontaneous'', ``to be efficient'', ``to be on time''.
Some fine-grained motives in the taxonomy could be merged. For instance, ``social group'' and ``close friends'', ``making friends'' and ``having close friends''.
Wherever possible, we further divide certain motives into sub-motives (``in love'' and ``in love with animal'' for instance), for more granularity.
Fig.~\ref{fig:ontology} illustrates our resulting ontology in full with hierarchy information and annotated image examples.


\begin{figure}
\centering
\includegraphics[width=\columnwidth]{images/annotation.pdf}
\caption{Annotation methods comparison. (a) A standard annotation process: given a image, choose the desired labels from a drop-down list; This approach is time-consuming and highly dependent on the expertise of annotators. (b) Our approach:  similarity comparison using ``unsatisfactory substitutes'' so the annotators can focus on the ``swapabilities'' of image pairs regarding the intent.
The task is to select all the images in the grid that clearly have a different intent than the reference image on the left. 
}
\label{fig:anno}
\vspace{-0.4cm}
\end{figure}


\cvpara{Annotation details}
Amazon Mechanical Turk (MTurk) was recruited to collect labels of perceived intent by employing a similarity comparison task that we call ``unsatisfactory substitutes''.
We rely on the notion of ``mental imagery''~\cite{sep-mental-imagery} -- a quasi-perceptual experience that maps example images to a visual representation in one's mind, along with \emph{games with a purpose}~\cite{von2006games, von2008recaptcha, deng2013fine, Horn2015} as our overall annotation approach.
Fig.~\ref{fig:anno} displays the differences between a standard annotation process and ours.
Due to space constraints, we leave other details in the Appendix~\ref{supsec:data}.


Although we have implemented strategies to ensure quality 
(see the Appendix~\ref{suppsubsec:anno_management}), 
we acknowledge that there are inevitable inconsistencies in our training data. 
Different people have different opinions of perceived intent.
Prior work~\cite{Horn2015} shows that there is at least 4\% error rate in popular datasets like CUB-200-2011~\cite{wah2011caltech} and ImageNet~\cite{imagenet_cvpr09}.
Yet these datasets are still effective for computer vision research.
Deep learning is robust to label noise in training set~\cite{Horn2015, rolnick2017deep}.
To this end, we create a highly curated test set by enlisting a single domain-specific taxonomic expert to provide the annotations for both validation (val) and test sets. In our experiments, we regard this expert's opinions as the ``gold standard,'' which allows us to focus on self-consistency in val and test sets, but we acknowledge that challenges remain in terms of resolving matters of disagreement among communities of experts. 
In the end, Intentonomy dataset has 12,740 training, 498 val, 1217 test images. 
Each image contains one or multiple intent categories.




==> main/sec4_content_exp.tex <==
\section{From Visual Content to Human Intent}
\label{sec:content_ana}


\begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{images/content_exp_compressed.pdf}
\caption{
Example images with full content (far left), and image modifications used for the controlled conditions of our study.
}
\label{fig:content_exps}
\vspace{-0.2cm}
\end{figure*}


Our goal is to investigate systematically how visual content within images contributes to the understanding of human intent.
To this end, we disentangle the impact of visual content on intent classification by a series of controlled experiments inspired by the methodology in~\cite{zhang2020puttingcontext}.
More specifically, we study the effect of visual content in terms of object ($\mathcal{O}$) and context ($\mathcal{C}$), and focus on the following fundamental aspects: (1) the amount of content information;
(2) three different content properties, including geometry, resolution, and low-level texture.
We then analyze the relationships between intent classes and specific things and stuff classes.
Fig.~\ref{fig:content_exps} and~\ref{fig:content_ana} provide an overview of our study under different control settings to analyze how visual information affects intent recognition.

More formally, given an image $I$, we apply a perturbation either to its objects or context to produce a modified image:
$I_x^{t} = f(I, t, x)$, $x \in \boldsymbol{X}, t \in \{\mathcal{O}, \mathcal{C}\}$,
where $f(\cdot)$ indicates a transformation function as will be introduced below and $\boldsymbol{X}$ is a set of positive integers defining the level of changes.
The larger the value of index $x$, the closer the $I_x^{t}$ is to the original images.
We now introduce different transformation functions used to see how intent recognition performance changes based on different visual contents.



\cvpara{Amount of content}
We control the amount of object or contextual information by expanding (or decreasing for context experiments) the bounding boxes (bbox) of detected objects by $e$ pixels:
\begin{equation*}
  I_x^{t} =
    \begin{cases}
      \text{bbox}^{t} & x = 0 \\
      \text{bbox$^{t}$ $\pm$ e}  & x \in [1 , 7]\quad e = 2^x  \\
      \text{full image}  & x = 8\\
    \end{cases}       
\end{equation*}
where bbox$^{(t \in \mathcal{O})}$ denotes the image area within the bounding box, and bbox$^{(t \in \mathcal{C})}$ is the area outside the bounding box (see two images in Fig.~\ref{fig:content_exps} (the third column from the right) for an example).
A total of 9 variations for both objects and context are included.
The larger $x$ indicates that the larger the amount of objects or context are presented. 



\begin{table}
\begin{center}
\resizebox{1.0\columnwidth}{!}{% 
\begin{tabular}{l c  c c   c}
\Xhline{1.0pt}\noalign{\smallskip}
Properties & $|\boldsymbol{X}|$  &$I_x^{t} = f(\cdot)$ \\
\Xhline{1.0pt}\noalign{\smallskip}

\texttt{Geometry}  & 6 & 
  $\text{jigsaw$_{(g \times g)}$}(t)$\eqcomma\\
 & &$g = 2^{5 - x}\eqcomma x \in [0, 5]$  \\
\hline\noalign{\smallskip}

\texttt{Resolution} &6 & $\text{blur$_{\sigma}$}(t),$\\
 & &$\sigma = 2^{5 - x}, x \in [0 , 5] $\\
\hline\noalign{\smallskip}

\texttt{Low-level} & 3 & \multirow{3}{*}{
    $\begin{cases}
      \text{no } $t$    & x = 0 \\
      \mathbbm{1} \{ \text{texture}(t) \} & x = 1, 2
    \end{cases} $}\\
\texttt{texture features} & & \\
 & &\\
\Xhline{1.0pt}\noalign{\smallskip}
\end{tabular}
}
\end{center}
\vspace{-0.3cm}
\caption{Content properties investigation. 
$t \in \{\mathcal{O}, \mathcal{C}\}$. 
}
\label{tab:content_prop}
\end{table}

\cvpara{Content properties}
We also study how visual properties impact intent recognition. 
We analyze the effect of the following properties of $\mathcal{O}$ and $\mathcal{C}$, including:\vspace{-0.3cm}\begin{enumerate}
    \setlength{\itemsep}{0pt}%
    \setlength{\parskip}{0pt}%
    \item \texttt{geometry}: regions of objects or context are broken down to $g \times g$ tiles and randomly re-arranged (we call this operation jigsaw), while the other content component remains intact;
    \item \texttt{resolution}: convolving the selected content component with a Gaussian function (zero-mean and various values of standard deviation $\sigma$);
    \item \texttt{low-level texture features}: visual textures are constructed using image statistics~\cite{portilla2000parametric} for the selected content component.
\end{enumerate}\vspace{-0.1cm}
For all three properties, we only modify the selected regions and paste other intact content components to their original locations. Table~\ref{tab:content_prop} describes our method in detail.



\begin{figure*}[t]
\centering
\subfigure[Content size.]{
    \includegraphics[scale=0.31]{images/fig_contentexp.pdf}
    \label{fig:bar_content}
}
% row 3
\subfigure[Content geometry.]{
    \includegraphics[scale=0.3]{images/ana_bar_jigsaw.pdf}
    \label{fig:bar_jigsaw}
}
\hfill
% bottom left 2
\subfigure[Content resolution.]{
    \includegraphics[scale=0.3]{images/ana_bar_blur.pdf}
    \label{fig:bar_blur}
}
\hfill
% bottom left 3
\subfigure[Content texture.]{
    \includegraphics[scale=0.3]{images/ana_bar_texture.pdf}
    \label{fig:bar_texture}
}

\caption{
A study on intent and content.
Overall there are three trends among 28 classes, which are presented in Figs.~\ref{fig:bar_content}-\ref{fig:bar_texture}. 
F1 scores, including average value and standard deviation over 5 runs, and random guess results, for selected classes and selected data variations are displayed. 
Class names ends with ``*'' are abbreviated (\eg ``Art-Arch*'' is short for ``appreciate architecture'').
}
\vspace{-0.3cm}
\label{fig:content_ana}
\end{figure*}


\cvpara{Analysis and discussion} 
Given each transformation $f$, we finetune a pretrained CNN model and obtain the macro F1 score on the modified validation set. Each model is run multiple times to reduce variance. Fig.~\ref{fig:content_ana} shows results of the 4 experiments focusing on content size and three properties.
In general, we observe a positive correlation between the amount of content and the macro F1 score. 
We can see in Fig.~\ref{fig:bar_content} that recognition F1 score decreases when context/object information is removed, for a majority of motive labels (\eg ``BeatCompete'' and ``SocialLife*''), confirming that context and objects clues are both important. 



Interestingly, there are some exceptions to this trend where either objects or context, on its own, yield comparable results to the original images. 
For categories like ``attractive'' or ``in love'', object information alone offers comparable F1-scores to full images. 
In other cases, contextual information achieves decent performance for motives like ``appreciate architecture'', ``natural beauty''.
Such motives are usually associated with representative gestures that provide strong supervisory signals (\eg, see Fig.~\ref{fig:teaser}). 
These signals usually come from single content module, which we further demonstrate in the next subsection.

In addition, Figs.~\ref{fig:bar_jigsaw}-\ref{fig:bar_texture} demonstrate how content properties affect intent recognition.
We see that geometry, blurred effect, and texture features of the content component decrease the intent recognition performance. 
See macro F1 score and ``beatCompete'' in Figs.~\ref{fig:bar_jigsaw}-\ref{fig:bar_texture} for example. Similar to the content size experiment previously, the impact of content properties is different for different classes.
The bottom plots of Figs.~\ref{fig:bar_jigsaw}-\ref{fig:bar_texture} show that ``Attractive'' is sensitive to object manipulation.
Motives like ``Art-Arch*'', on the other hand, have an opposite trend where context contributes more than objects. The recognition results are robust to object manipulation, yet sensitive to context modulation overall.
These observations are further illustrative of the varying importance of objects or contextual information for different classes.




\begin{figure}
\includegraphics[width=0.95\columnwidth]{images/cam_intent_content_softlog_compressed.pdf}
\caption{
A visualization of $\Pi$ (Eq.~\ref{eq:cor}), where each entry denotes the correlation between a pair of intent and object/context class.
}
\vspace{-0.4cm}
\label{fig:cam_ana}
\end{figure}


\cvpara{Relationship between intent and object/context classes} 
The above analysis demonstrates different intent categories have different preferences on objects and/or context. We now examine whether there exists relationships between intent categories and
\emph{specific} objects/context classes. 


More specifically, given an image $I$ with a intent label $m$ and a trained intent recognition model,  we use class activation mappings~\cite{zhou2015cnnlocalization}, to produce a binary mask $\text{CAM}^{b}(I, m, \tau_{cam})$ ($\tau_{cam}$ is a threshold value) to represent the discriminate image regions for class $m$ in the image. We also feed the image to a segmentation model pretrained on the COCO Panoptic dataset~\cite{kirillov2019panoptic} to obtain a binary mask $\text{Pano}(I, p, \tau_p)$ ( $\tau_p$ is a threshold value) for the class $p$ in the COCO dataset. We use the COCO Panoptic dataset~\cite{kirillov2019panoptic} because it contains widely used  \textit{thing} and \textit{stuff} categories. We then define the correlation between $p$ and $m$ as:
\begin{equation}
    \label{eq:cor}
\Pi_{p, m}  = \frac{\text{CAM}^{b}(I, m, \tau_{cam}) \cap \text{Pano}(I, p, \tau_p)}{\text{Pano}(I, p, \tau_p)}\eqdot
\end{equation}


Here, objects with high scores tend to
be semantically meaningful for the corresponding intent categories.
Fig.~\ref{fig:cam_ana} further validates our findings in the content modulation experiments.
While there are intent classes requiring both object and context, certain classes are object-oriented while others are context-oriented.
Further, it can be observed that certain intent classes are also more dependent on particular object or context classes. 
For example, ``person'' is semantically meaningful for intent like ``Attractive'' and ``inHarmony''.
It is also consistent that stuff classes like ``building'', ``bridge'' can help discriminate classes like ``Architecture''.


It is worth mentioning that some intent classes (\eg ``easyLife'', ``socialLife'') have no or few correlated thing or stuff classes.
Indeed, the F1 score for some motive classes are comparable to random guessing (see Fig.~\ref{fig:bar_content}). 
We suspect that visual information only is not enough to represent the inherent visual and semantic diversity in those classes.


==> main/sec5_0_overview.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{images/fig_method_compressed.pdf}
\caption{Method overview. Given an image $I$, we localize important object and context regions for an intent of interest and additionally use hashtags to complement visual information. See texts for more details.
}
\label{fig:model_all}
\end{figure*}

\section{Multimodal Intent Recognition}
\label{sec: method}

The study in Sec.~\ref{sec:content_ana} demonstrates that different intent classes have different correlation with context and objects, and so using a single ``one-size-fits-all'' network for intent recognition is sub-optimal. To mitigate this issue, we introduce a localization loss that identifies, for each class, regions in images that are important (Sec.~\ref{subsec:cam_method}).
In addition, as shown, visual information alone is not sufficient for predicting certain classes of intent. To compensate, we also propose to use an auxiliary channel to provide complementary semantic information (Sec.~\ref{subsec:hs_method}).
The overall framework is presented in Fig.~\ref{fig:model_all}.



==> main/sec5_1_cam.tex <==
\subsection{Object/Context localization}\label{subsec:cam_method}

Since different intent classes rely on different visual content (either $\mathcal{O}$ or $\mathcal{C}$), we wish to guide the network to attend to these regions when recognizing a class of interest. In particular, we first split all intent categories into 3 groups based on our study in Sec.~\ref{sec:content_ana}: object-dependent ($M_{\mathcal{O}}$), context-dependent ($M_{\mathcal{C}}$ ), and others which depends on the entire image.
We then use CAM~\cite{zhou2015cnnlocalization} to localize salient regions in a weakly-supervised manner and minimize the overlap area between CAM and the image area that is not a region of interest (Fig.~\ref{fig:model_all}).


Formally, given a motive class $m$ and an image sample $I$, $\text{CAM}(I, m)$ denotes the real-valued version of $\text{CAM}^{b}(I, m, \tau_{cam})$ (see Sec.\ref{sec:content_ana}).
Let $\text{Mask}^{\mathcal{C}}(I)$ and $\text{Mask}^{\mathcal{O}}(I)$ be the aggregated binary masks in image $I$ that represent all detected thing ($P_{\mathcal{T}}$) and stuff classes ($P_{\mathcal{S}}$), respectively.
See examples of $\text{Mask}^{\mathcal{O}}(I)$ and $\text{Mask}^{\mathcal{C}}(I)$ in Fig.~\ref{fig:model_all}.
The localization loss is then defined as:
\begin{align}
  L^{\mathcal{O}} &=\sum_{m \in M_{\mathcal{O}}} \left(\text{CAM}(I, m) \odot \text{Mask}^{\mathcal{C}} (I)  \right)\eqcomma  \label{eq: cam_loss_o}  \\
  L^{\mathcal{C}} &=\sum_{m \in M_{\mathcal{C}}} \left(\text{CAM}(I, m) \odot \text{Mask}^{\mathcal{O}} (I)  \right)\eqcomma \label{eq: cam_loss_c}
\end{align}
where $\odot$ is element-wise multiplication. The final loss $\mathcal{L}_{loc}$ is the summation of all the entries in $L^{\mathcal{O}}$ and $L^{\mathcal{C}}$.



Note that our approach is similar to previous work that addresses contextual bias~\cite{singh-cvpr2020}.
Both approaches use CAM as weak annotations to guide training.
However, our method does not require a regularization term which grounds CAMs of each category to be closer to the regions from a previously trained model.
Therefore, our approach can be trained with a single pass, in an end-to-end fashion.


==> main/sec5_2_hs.tex <==
\subsection{Hashtags as an auxiliary modality}\label{subsec:hs_method}

Visual information is not sufficient for recognizing certain intent categories~(see ``EasyLife'' in Fig.~\ref{fig:cam_ana}). To further improve intent recognition, we resort to language information as a complementary clue for improved performance. Unfortunately, images from Unsplash are not associated with any text information. We instead leverage visual similarities of the Unsplash images to a larger set of images, which do contain associated metadata that loosely describe the semantics within the images. Instagram (IG) is a social media platform that contains billions of publicly available photos, often with user-provided hashtags. This presents an opportunity to weakly relate images with vastly different visual appearances that contains similar semantic information, by means of hashtags.

In particular, we first compute regional maximum activations of convolutions features~\cite{GordoARL16,tolias2016particular} from the last activation map of a pretrained Resnext-50 (32x4) model (trained on ImageNet-22k~\cite{imagenet_cvpr09}) on 7-days of public photos from IG as well as all the images from our intent dataset. 
Using these embeddings, we then perform a KNN query for each Unsplash image to retrieve the top $k$ matching IG images for each of the images in our intent dataset.
Finally, for each matching IG photo, we collect all of the associated hashtags (additional details are in the supplemental material).
The collection of all matched hashtags for a given Unsplash image are represented as an unordered set $\boldsymbol{HT}$.
See Fig.~\ref{fig:model_all} for examples of fetched hashtags.
However, directly using hashtags are challenging because: 1) hashtags can be noisy, much like web-scale data tends to be; 2) a hashtag is usually a concatenation of several words, including multilingual phrases and emojis (\eg \hs{coffeme}, \hs{landscapephotography}).
There are a large amount of out of vocabulary words if one uses a pre-trained word embedding for the entire hashtag.
We thus first break the hashtags down using a known dictionary of words (\ie \hs{coffeeme} $\rightarrow$ ``coffee'' ``me''). Subsequently, unusual and noisy tokens/hashtags are automatically filtered out.

Formally, given $\boldsymbol{HT}$ for one image sample and a dictionary $\mathcal{V}$, we first segment each hashtag $hs$ into a list of tokens based on the given vocabulary: $\text{WordBreak}(hs, \mathcal{V}) = [w]$, $w\in \mathcal{V}$, $hs \in \boldsymbol{HT}$. 
Separated tokens of one hashtag are mapped to a dense embedding individually, and aggregated into a single representation.
Next, all of the resulting hashtag representations are averaged to compute a unified feature for all hashtags associated with a single image.
Finally, the hashtag features are concatenated with image features into an integrated representation for classification.






\cvpara{Loss function}
To capture the different opinions from crowd annotators, we use cross-entropy loss with soft probability, denoted as $\mathcal{L}_{CE}$, inspired by~\cite{wslimageseccv2018}\footnote{Similar to~\cite{wslimageseccv2018}, we also tried sigmoid cross-entropy loss but obtained worse results.}.
More formally, our model computes probabilities $\hat{\boldsymbol{y}}^{intent}$ using a softmax activation, and minimizes the cross-entropy between $\hat{\boldsymbol{y}}^{intent}$ and the target distribution $\boldsymbol{y}^{intent}$.
$\boldsymbol{y}^{intent}$ is a target vector, where each position $m$ contains the number of crowd workers who labeled the associated image to motive class $m$, normalized by the total number of crowd workers to indicate a probability distribution.


% When the localization loss $\mathcal{L}_{loc}$ is applied, we sum both $\mathcal{L}_{loc}$ and $\mathcal{L}_{CE}$: 
% % The final loss of training the multimodal framework is defined as the sum of the cross entropy loss $\mathcal{L}_{CE}$ and the localization loss $\mathcal{L}_{loc}$: 
% $\mathcal{L} = \lambda \mathcal{L}_{loc} + \mathcal{L}_{CE}$. $\lambda$ is a scalar to determine the contribution of each loss term.
% % Then the localization loss $\mathcal{L}_{loc}$ is summed with the cross entropy loss $\mathcal{L}_{CE}$.
% % \begin{equation}
% %     \label{eq: all_loss}
% %     \mathcal{L} = \lambda \mathcal{L}_{loc} + \mathcal{L}_{CE}
% % \end{equation}




% Formally,
% \begin{equation}
% \label{eq: hs_embd}
%     g(\theta(\text{WordBreak}(hs, \mathcal{V}))
% \end{equation}
% Then two additional learnable fully connected (FC) layers are added
% to map the the unified embedding into the common space with dimension $D$.

% fusion techniques: Sum, concat, max, mean: concat works best
% Hashtag topk: k: 30 works best than {25,  50,  75, 100, 150, 200, 250} 
% Hashtags: 
% mean instead of sum (  {[w1 w2], [w3], [w4 w5 w6]}  -> mean([mean([bert(w1) bert(w2)]), bert(w3), mean([bert(w4) bert(w5) bert(w6)])]) )
% Remove emoji: not helping;
% Add none-breakable hashtags words: not helping
% Hashtags embeddings (TBC): static bert works best? Than glove? 
% Losses: cross-entropy with soft probability works best


==> main/sec6_1_results_main.tex <==
\section{Experiments}
\label{sec: exp}
In this section, we conduct extensive experiments to evaluate the effectiveness of different components of the multimodal framework. More specifically, we report the performance of the following approaches: (1) \textsc{Random}, which is the success rates by random guessing; (2) \textsc{Visual}, which finetunes a standard ResNet50 model to classify motives; (3) \textsc{Hashtags} (\textsc{ht}), which only uses hashtags to predict intent; (4) \textsc{Visual} + \textsc{ht}, which combines visual information and hashtags; (5) \textsc{Visual} + $\mathcal{L}_{loc}$, which augments a visual model with the proposed localization loss; (6) \textsc{Visual} + $\mathcal{L}_{loc}$ + \textsc{ht}, which denotes our full model. Among them, (2)-(4) are trained using the standard cross-entropy loss only, $\mathcal{L}_{CE}$. 
When the localization loss $\mathcal{L}_{loc}$ is applied, we sum both $\mathcal{L}_{loc}$ and $\mathcal{L}_{CE}$: 
$\mathcal{L} = \lambda \mathcal{L}_{loc} + \mathcal{L}_{CE}$. $\lambda$ is a scalar to determine the contribution of each loss term.
Performance are measured using Macro F1, Micro F1, and Samples F1 scores. We repeat each experiment 5 times and report the mean and standard deviation (std).

\input{main/table_mainresult}
\input{main/table_subsets_long}



Table~\ref{tab: f1s_all} summarizes the results. We can see that the full model achieves a 31.12 macro F1 score, outperforming the \textsc{Visual} baseline by +7.76\% percent difference, as well as the \textsc{ht} baseline by +57.81\% percent difference. 
Furthermore, compared to the \textsc{Visual} only approach, adding the localization loss improves macro F1 score by 5.16\%. We also observe that visual and text information are complementary, offering 4.99\% and 53.75\% gain compared to visual and text only, respectively.


To better understand why $\mathcal{L}_{loc}$ and \textsc{ht} improve visual only model, we break down the intent classes into different subsets based on their content dependency, \ie, object-dependent ($\mathcal{O}$-classes), context-dependent ($\mathcal{C}$-classes), and \emph{Others} which depends on both foreground and background information; (2) difficulty, which measures how much the \textsc{Visual} outperforms achieves than the \textsc{Random} results (``easy'', ``medium'' and ``hard'').
More details are given in the Appendix~\ref{supsec:model}.
Table~\ref{tab:f1s_contentdiff} summarizes the subset results.



==> main/sec6_2_results_loc.tex <==
\cvpara{The effectiveness of $\mathcal{L}_{loc}$}
We see from Table~\ref{tab:f1s_contentdiff} that when adding the localization loss gains are more significant for $\mathcal{O}$-classes, compared to $\mathcal{C}$-classes and \emph{Others}.
The localization loss depends on the area of either object or context regions in the images, and the  objects' region, which is used in $\mathcal{L}^{\mathcal{C}}$ in Eq.~\ref{eq: cam_loss_c}, are typically small\footnote{Note that  $\mathcal{L}^{\mathcal{C}}$ minimizes the overlap region between object area and the salient region (CAM).}.
As a result, the $\mathcal{L}_{loc}$ has no significant effect on the final score. 




We also conduct a qualitative study to understand why the localization loss helps intent recognition. Results are shown in Fig.~\ref{fig:cam_vis}. We can see that the localization loss helps the model to focus on the correct region of interest for both $\mathcal{O}$- and $\mathcal{C}$-classes, especially when the image is scattered with multiple objects and scenes. 
Fig.~\ref{fig:cam_vis}(a) confirms that \textsc{Visual} + $\mathcal{L}_{loc}$ works well when both object and context information are presented in the image (bottom 2 examples), or the target region of interest is small (top example).
We also note in Fig.~\ref{fig:cam_vis}(b) that for images where the region of interest is located in the center, or is relatively large, both \textsc{Visual} and our method give good results.



==> main/sec6_3_results_hs.tex <==
\cvpara{The effectiveness of hashtags}
From Table~\ref{tab:f1s_contentdiff}, we observe that the model using both images and hashtags outperforms the uni-modal approaches over ``easy'' and ``hard'' classes, without hurting the ``medium'' classes. 
This suggests there is value in the auxiliary information to help close the semantic gap.
Therefore, our results suggest that images and hashtags do in fact complement each other in the motive recognition task.
For example, \hs{love} is directly indicative of the intent label ``in love'', as is \hs{workout} of ``health'' (see Fig.~\ref{fig:model_all} for more hashtag examples).
Interestingly, for ``easy'' classes, \textsc{ht} model outperforms the \textsc{Visual} model by 8.2\%, however it struggles with the ``medium'' and ``hard'' classes (Table~\ref{tab:f1s_contentdiff}).
This suggests that hashtags provided by users, while noisy, do still contain information about intent to some extent.




It is perhaps counter-intuitive that hashtags do not outperform visual signals entirely.
While hashtags seem to capture the essence of human intents (see examples in Fig.~\ref{fig:model_all}), 
careful inspection of the fetched hashtags shows that not all hashtags are useful in practice. Obscurity and ambiguity exist, including typos, slang, inside jokes, and irrelevant information. 
More effective modeling of hashtags remains an open research problem.


==> main/table_mainresult.tex <==
\begin{table}[t]
\begin{center}
\resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{ l c c c }
\Xhline{1.0pt}\noalign{\smallskip}
\textbf{Method} & \textbf{Macro F1} & \textbf{Micro F1} & \textbf{Samples F1}  \\ 
\Xhline{1.0pt}\noalign{\smallskip}
\textsc{Random} &      \meanstd{6.94}{0.09}   & \meanstd{7.18}{0.10}   &\meanstd{7.10}{0.10} \\
\hline\noalign{\smallskip}

\textsc{Visual}   & \meanstd{28.88}{0.56} & \meanstd{37.08}{1.07}  &\meanstd{36.06}{1.51} \\
 \noalign{\smallskip}

\textsc{ht}   &\meanstd{19.72}{0.88}   &\meanstd{29.30}{1.62}           &\meanstd{31.47}{1.64}\\
\hline\noalign{\smallskip}

\multirow{2}{*}{\textsc{Visual} + $\mathcal{L}_{loc}$}    &\meanstd{30.37}{0.51} &\textbf{\meanstd{38.64}{0.95}}	& \meanstd{37.41}{1.51}   \\
 &   \small{(\textcolor{green_im}{+1.49})}   & \small{ (\textcolor{green_im}{+1.56} )}  & \small{(+1.35)}  \\

 \hline\noalign{\smallskip}

\textsc{Visual}  &\meanstd{30.32}{0.62}	 &\meanstd{37.61}{0.85}	&\textbf{\meanstd{38.98}{1.70}}   \\
+ \textsc{ht} &   \small{(\textcolor{green_im}{+1.44}) }   & \small{(+0.53)}  &\small{ (\textcolor{green_im}{+2.92}) } \\
 \hline\noalign{\smallskip}
 
\textsc{Visual} + $\mathcal{L}_{loc}$ &\textbf{\meanstd{31.12}{0.63}}  &\meanstd{38.49}{0.88}	&\meanstd{38.77}{1.74}
  \\
+ \textsc{ht} &  \small{(\textcolor{green_im}{+2.24})}
&  \small{(\textcolor{green_im}{+1.41})}   &  \small{(\textcolor{green_im}{+2.71}) }\\

\Xhline{1.0pt}\noalign{\smallskip}
\end{tabular}
}
\caption{Experimental results of different approaches for intent recognition measured in Micro F1, Macro F1, Samples F1 scores.
(+ $\cdot$) indicate the difference comparing to \textsc{Visual}. \textcolor{green_im}{(+ $\cdot$) in green} denotes that the difference is larger than the std.}
\vspace{-0.4cm}
\label{tab: f1s_all}
\end{center}
\end{table}



==> main/table_subsets_long.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{ l l l  l  l l l}
\Xhline{1.0pt}\noalign{\smallskip}
\textbf{Method}  & \multicolumn{3}{ c }{\textbf{Content}}  & \multicolumn{3}{ c }{\textbf{Difficulty}}  \\
\cline{2-7}\noalign{\smallskip}
& $\mathcal{O}$-classes & $\mathcal{C}$-classes & \emph{Others}     & Easy & Medium & Hard   \\ 
\Xhline{1.0pt}\noalign{\smallskip}

\textsc{Random}    &\meanstd{7.75}{5.47}  &\meanstd{12.53}{5.96} &\meanstd{6.05}{5.23}
            & \meanstd{19.86}{1.28} & \meanstd{7.11}{3.40} & \meanstd{2.81}{1.80} \\
\hline\noalign{\smallskip}
\textsc{Visual} & \meanstd{34.92}{3.63}   & \meanstd{41.27}{3.53}  &  \meanstd{25.34}{1.13}
            & \meanstd{61.84}{4.90}	 & \meanstd{33.71}{2.24}  &\meanstd{11.73}{1.74}\\
            
\textsc{ht}  &\meanstd{26.96}{0.80}  &\meanstd{35.15}{4.18}   & \meanstd{15.43}{0.87}
&\meanstd{63.58}{1.79}	& \meanstd{19.68}{1.70} & \meanstd{6.63}{1.43}\\

\hline\noalign{\smallskip}

\textsc{Visual} + $\mathcal{L}_{loc}$  &\meanstd{38.82}{1.95}\small{(\textcolor{green_im}{+3.9})}  
&\meanstd{\textbf{43.14}}{3.00} \small{(+1.87)}
&\meanstd{25.90}{1.35}\small{(+0.56)}
&\meanstd{63.67}{1.47}\small{(+0.09)} 
&\meanstd{\textbf{34.72}}{1.26} \small{(+1.01)}& \meanstd{13.83}{1.13}\small{(\textcolor{green_im}{+2.10}) }\\

\hline\noalign{\smallskip}

\textsc{Visual} + \textsc{ht}
  & \meanstd{37.71}{2.70} \small{(+2.79)}  &\meanstd{42.17}{3.62} \small{(+0.90)} & \meanstd{26.36}{1.17} \small{(+1.02) }
  &\meanstd{\textbf{66.67}}{2.12} \small{(+4.83)} &\meanstd{32.93}{1.57}\small{(-0.78)}	&\meanstd{15.52}{0.98} \small{(\textcolor{green_im}{+3.79})}\\
 
\hline\noalign{\smallskip}

\textsc{Visual} + $\mathcal{L}_{loc}$ + \textsc{ht}
&\meanstd{\textbf{39.82}}{1.56}	\small{(\textcolor{green_im}{+4.90}) } 
&\meanstd{42.09}{2.57} \small{(+0.82)}
&\meanstd{\textbf{26.77}}{1.13} \small{(\textcolor{green_im}{+1.43})}
&\meanstd{66.18}{4.56}	\small{(+4.34)}
&\meanstd{33.86}{1.08}	\small{(+0.15)}
&\meanstd{\textbf{16.50}}{1.80} \small{(\textcolor{green_im}{+4.77})} \\

\Xhline{1.0pt}\noalign{\smallskip}
\end{tabular}
}
\caption{Experimental results 
in terms of how much object/context information intent categories need (content), and how difficult it is for \textsc{VISUAL} to outperforms the \textsc{Random} results (difficulty).
(+ $\cdot$) indicates the difference comparing to \textsc{Visual}. \textcolor{green_im}{(+ $\cdot$) in green} denotes that the difference is larger than the std.
}
\vspace{-0.4cm}
\label{tab:f1s_contentdiff}
\end{center}
\end{table*}

\begin{figure*}[t!]
\centering
\includegraphics[width=0.92\linewidth]{images/fig_results.pdf}
\caption{
Analysis of the proposed localization loss.
(a) \textsc{Visual} + $\mathcal{L}_{loc}$ approach learns to isolate appropriate regions of interest, comparing to \textsc{visual}.
For example, our method learn to focus on the dog and girl respectively for ``In love (animal)'' and ``Attractive'' respectively, which are $\mathcal{O}$-classes.
(b) Examples for which both \textsc{visual} + $\mathcal{L}_{loc}$ and \textsc{visual} produce similar visualizations. Both methods focus on the correct region, which are located in center and account for a larger area of the image.
}
\label{fig:cam_vis}
\end{figure*}
